A CLIP-Hitchhiker's Guide to Long Video Retrieval

Our goal in this paper is the adaptation of image-text models for long video retrieval. Recent works have demonstrated state-of-the-art performance in video retrieval by adopting CLIP, effectively hitchhiking on the image-text representation for video tasks. However, there has been limited success in learning temporal aggregation that outperform mean-pooling the image-level representations extracted per frame by CLIP. We find that the simple yet effective baseline of weighted-mean of frame embeddings via query-scoring is a significant improvement above all prior temporal modelling attempts and mean-pooling. In doing so, we provide an improved baseline for others to compare to and demonstrate state-of-the-art performance of this simple baseline on a suite of long video retrieval benchmarks.

==> tables/anet.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}
\centering
\scriptsize
\caption{Text-to-video retrieval results on the ActivityNet Captions test set.}
\begin{tabular}{@{}lcrrrrr@{}}
\toprule
\textbf{Method}  & agg. & \textbf{R@1}  & \textbf{R@5}  & \textbf{R@10} & \textbf{MedR} & \textbf{MnR} \\ \midrule
Frozen & ST$_{attn}$& 28.8          & -         & 60.9       & 3.0 & -         \\
CLIP4CLIP & mean & 40.5        & 72.4         & -       & 2.0    & 7.4       \\
CLIP4CLIP & seqTransf & 40.5       & 72.4        & -       & 2.0 & 7.5          \\
\midrule

Ours & Q-score  & \textbf{44.0} & \textbf{74.9} & \textbf{86.1} & 2.0 &  \textbf{5.8} \\ \bottomrule
\end{tabular}
\label{tab:anet-sota}
\end{table}
